Self-Consuming Generative Models Go MAD

Seismic advances in generative AI algorithms for imagery, text, and other data types has led to the temptation to use synthetic data to train next-generation models. Repeating this process creates an autophagous (self-consuming) loop whose properties are poorly understood. We conduct a thorough analytical and empirical analysis using state-of-the-art generative image models of three families of autophagous loops that differ in how fixed or fresh real training data is available through the generations of training and in whether the samples from previous generation models have been biased to trade off data quality versus diversity. Our primary conclusion across all scenarios is that without enough fresh real data in each generation of an autophagous loop, future generative models are doomed to have their quality (precision) or diversity (recall) progressively decrease. We term this condition Model Autophagy Disorder (MAD), making analogy to mad cow disease.

==> Fully_Synthetic_unbiased_figures.tex <==
%% --------------------------------------
%% Synthetic unBiased
%% FID, Precision, Recall Plots
%% --------------------------------------


\begin{figure}[t]

\centering
\begin{tikzpicture}
    
\pgfplotLL

\pgfplotsset{/pgfplots/group/every plot/.append style = {
    very thick, no markers
}};

\begin{groupplot}[group style = {group size = 3 by 1, horizontal sep = 30pt}, width = 0.36\linewidth]%, height = 5.0cm]

    
    \nextgroupplot[
        title = {},
        xmax=5,
        ylabel={\small FID},
        xlabel={\small Number of Generations},
        axis x line*=bottom,
        axis y line*=left,
        grid,
        legend style = { nodes={scale=0.7, transform shape},column sep = 10pt, legend columns = -1, legend to name = grouplegend1, text=black, cells={align=left},}]

        \addplot
        table [
            x index=0, 
            y index=1, 
            col sep=comma] {csv/ffhq/ffhq_fid_so.csv};

        \addplot
        table [
            x index=0, 
            y index=1, 
            col sep=comma] {csv/mnist_diff/MNIST_full_fid.csv};

        \addlegendentryexpanded{StyleGAN2 on FFHQ $\bias = 1$};
        \addlegendentryexpanded{DDPM on MNIST $\bias = 1$};
        
        

    \nextgroupplot[
        title = {},
        xmax=5,
        ylabel={\small Precision},
        xlabel={\small Number of Generations},
        axis x line*=bottom,
        axis y line*=left,
        grid]

        \addplot
        table [
            x index=0, 
            y index=1, 
            col sep=comma] {csv/ffhq/ffhq_precision_so.csv};

        \addplot
        table [
            x index=0, 
            y index=1, 
            col sep=comma] {csv/mnist_diff/MNIST_full_precision.csv};


    \nextgroupplot[
        title = {},
        xmax=5,
        ylabel={\small Recall},
        xlabel={\small Number of Generations},
        axis x line*=bottom,
        axis y line*=left,
        grid]
        
        \addplot
        table [
            x index=0, 
            y index=1, 
            col sep=comma] {csv/ffhq/ffhq_recall_so.csv};

        \addplot
        table [
            x index=0, 
            y index=1, 
            col sep=comma] {csv/mnist_diff/MNIST_full_recall.csv};


\end{groupplot}
\node at ($(group c2r1) + (0,-85pt)$) {\ref{grouplegend1}}; 

\end{tikzpicture}

\caption{\textbf{Training generative models on only synthetic data without sampling bias always reduces the quality and diversity of synthetic data.} The FID (left), quality (precision, middle), and diversity (recall, right) of synthetic FFHQ and MNIST images produced in their own synthetic-training loops. }
\label{fig:synthetic_unbiased_fid_precision_recall}

\end{figure}


\begin{figure}[t]
    \centering % <-- added
    \foreach \b in {2,5,10}{
    \begin{minipage}{0.25\linewidth}
    \centering
  \includegraphics[width=\linewidth]{./img/tsnedata_generation\b_w0.jpg} \\ \small Generation \b
  \end{minipage}
  }
\caption{\small here goes caption }


\label{fig:tsne1}
\end{figure}

==> hb_diagram.tex <==
%\documentclass[10pt]{article}

%\usepackage{tikz}

%\usetikzlibrary{decorations.text, fit, positioning, shapes.geometric}

%\pagestyle{empty}
%\begin{document}




% Based on pgfplots Dark2
%\definecolor{colorA}{HTML}{1B9E77}
%\definecolor{colorB}{HTML}{D95F02}
%\definecolor{colorC}{HTML}{7570B3}
%\definecolor{colorD}{HTML}{E7298A}


%\def\bias{r}






\begin{tikzpicture}

\definecolor{textColor}{HTML}{000000};
\def\opacity{70};

\def\diamondsize{1cm};
\def\minidiamondsize{0.5\diamondsize};

\def\xdist{0.75cm};
\def\ydist{1cm};

\def\rectheight{0.75cm};


%% ----------------
%% Geometric Shapes
%% ----------------

% Rectangle: Fixed Real Data
\node[rectangle, draw,
    text=textColor, fill=colorB!\opacity,
    minimum width=3cm, minimum height=\rectheight] 
    (fixed_real) {Fixed Real Data};

% Diamond: Data 0
\node[diamond, draw, text = textColor,
    fill = colorB!\opacity, minimum size=\diamondsize,
    above=\ydist-0.25cm of fixed_real.north west]
    (data0) {Data 0};
    
% Rectangle: Model 1
\node[rectangle, draw,
    text=textColor, fill=colorA!\opacity,
    minimum width=2cm, minimum height=\rectheight,
    right=\xdist of data0.east, anchor=west]
    (model1) {Model 1};

% Diamond: Data 1
\node[diamond, draw, text = textColor,
    fill = colorA!\opacity, minimum size=\diamondsize,
    right=\xdist of model1.east, anchor=west]
    (data1) {Data 1};

\node[diamond, draw,
    fill = colorC!\opacity, minimum size=\minidiamondsize,
    below= 0cm of data1.north, anchor=north]
    {};

\node[diamond, draw,
    fill = colorB!\opacity, minimum size=\minidiamondsize,
    below= 0cm of data1.south, anchor=south]
    {};

% Rectangle: Fresh Data 1
\node[rectangle, draw,
    text=textColor, fill=colorC!\opacity,
    minimum width=3cm, minimum height=\rectheight,
    above=\ydist of data1.north, anchor=south]
    (fresh1) {Fresh Real Data};

% Rectangle: Model 2
\node[rectangle, draw,
    text=textColor, fill=colorA!\opacity,
    minimum width=2cm, minimum height=\rectheight,
    right=\xdist of data1.east, anchor=west]
    (model2) {Model 2};

% Diamond: Data 2
\node[diamond, draw, text = textColor,
    fill = colorA!\opacity, minimum size=\diamondsize,
    right=\xdist of model2.east, anchor=west]
    (data2) {Data 2};

\node[diamond, draw,
    fill = colorC!\opacity, minimum size=\minidiamondsize,
    below= 0cm of data2.north, anchor=north]
    {};

\node[diamond, draw,
    fill = colorB!\opacity, minimum size=\minidiamondsize,
    below= 0cm of data2.south, anchor=south]
    {};

% Rectangle: Fresh Data 2
\node[rectangle, draw,
    text=textColor, fill=colorC!\opacity,
    minimum width=3cm, minimum height=\rectheight,
    above=\ydist of data2.north, anchor=south]
    (fresh2) {Fresh Real Data};

% Ellipses
\node[right=0.25cm of data2] {\LARGE\ldots};


%% ------
%% Arrows
%% ------

% Real Data
\draw[dotted, colorB!\opacity,
    line width=2pt, -latex]
    (fixed_real.north west) -- (data0);

\draw[dotted, colorB!\opacity,
    line width=2pt, -latex]
    (fixed_real.east) to[out=0, in=-90] (data1.south);

\draw[dotted, colorB!\opacity,
    line width=2pt, -latex]
    (fixed_real.east) to[out=0, in=-90] (data2.south);

% Training + Generating Data
\draw[colorA!\opacity, line width=2pt, -latex,
    postaction={decorate,decoration={raise=1ex,text along path,text align=center,text={Trains}}}
    ] (data0) to[out=45,in=135] (model1);

\draw[colorA!\opacity, line width=2pt, -latex,
    postaction={decorate,decoration={raise=3.2ex,text along path,text align=center,text={Samples}}},
    postaction={decorate,decoration={raise=1ex,text along path,text align=center,text={w/ bias $\bias$}}}
    ] (model1) to[out=45, in=135] (data1);

\draw[colorA!\opacity, line width=2pt, -latex,
    postaction={decorate,decoration={raise=1ex,text along path,text align=center,text={Trains}}}
    ] (data1) to[out=45, in=135] (model2);

\draw[colorA!\opacity, line width=2pt, -latex,
    postaction={decorate,decoration={raise=3.2ex,text along path,text align=center,text={Samples}}},
    postaction={decorate,decoration={raise=1ex,text along path,text align=center,text={w/ bias $\bias$}}}
    ] (model2) to[out=45, in=135] (data2);

% Fresh Data
\draw[dotted, colorC!\opacity,
    line width=2pt, -latex]
    (fresh1) -- (data1.north);

\draw[dotted, colorC!\opacity,
    line width=2pt, -latex]
    (fresh2) -- (data2.north);



\end{tikzpicture}







%\end{document}
